Emotional Musical Prosody for the Enhancement of Trust in Robotic Arm Communication

As robotic arms become prevalent in industry it is crucial to improve levels of trust from human collaborators. Low levels of trust in human-robot interaction can reduce overall performance and prevent full robot utilization. We investigated the potential benefits of using emotional musical prosody to allow the robot to respond emotionally to the user's actions. We tested participants' responses to interacting with a virtual robot arm that acted as a decision agent, helping participants select the next number in a sequence. We compared results from three versions of the application in a between-group experiment, where the robot had different emotional reactions to the user's input depending on whether the user agreed with the robot and whether the user's choice was correct. In all versions, the robot reacted with emotional gestures. One version used prosody-based emotional audio phrases selected from our dataset of singer improvisations, the second version used audio consisting of a single pitch randomly assigned to each emotion, and the final version used no audio, only gestures. Our results showed no significant difference for the percentage of times users from each group agreed with the robot, and no difference between user's agreement with the robot after it made a mistake. However, participants also took a trust survey following the interaction, and we found that the reported trust ratings of the musical prosody group were significantly higher than both the single-pitch and no audio groups.

==> spare.tex <==

% % %http://www0.cs.ucl.ac.uk/research/researchnotes/documents/RN_04_19_000.pdf
% % %https://www.tandfonline.com/doi/full/10.1080/00140139.2018.1457725?af=R
% % General trust and methods for recovery

% % % communicating intent https://www.sciencedirect.com/science/article/pii/S1389041716301802
% % % more intent https://dl.acm.org/doi/10.1145/2696454.2696475

% % % TAN TEST - http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.248.8068&rep=rep1&type=pdf


% % ARM ASSISTANCE WITH A TASK, - the arm can show emotion...
% % --- sorting task, sorting good from bad! so much better, this is a real task. 

% % Papers in trust experiment



\subsection{Robotic Arm Forms of Communication}
Amongst research into methods for robotic arms to communicate and signal their intent, there is no standardized set of approaches \cite{cha2018survey}. In social robotics communication is often derived from human behaviour - such as gestures and gaze - these are not however readily available to robotic arms \cite{rosen2019communicating}. Additionally when these forms of communication are added to arms they require significant expense, such as extra visual displays like a face\cite{6839819}, or in the case of added gestures risk challenging and reducing the core functionality of the arm. In robotic research, forms of non-verbal communication can generally be split into four categories kinesics, proxemics, haptics and chronemics, none of which are easily applied to an existing robotic system \cite{saunderson2019robots}. While varying movement to show intent has shown successful results \cite{bodden2016evaluating}, changes to path planning and movement dynamics is often not feasible. Another effective method for arms to display their intent is through vision of a robot's future trajectory, such as by a human worn head mounted display \cite{ruffaldi2016third}, however this requires a significant investment and potential distraction to the user.  Emotion has been more commonly used as an input to robotic arms, such as facial emotion recognition to control and change the behaviour of robotic arms \cite{mei2016emotion,iengo2012attentional,ying2016emotion}. Likewise, GSR emotional evaluation on humans has been used to impact a robot's control pattern \cite{takahashi2001human}. Nevertheless, robotic arm displays of emotion in work and collaboration, or interaction beyond showing intent are widely overlooked in robotics literature. 


\subsection{Communication for Trust and Trust Recovery}
For collaboration with robotic arms trust is required, without which they can be underutilized \cite{johndlee}. Trust is largely developed in the first phase of a relationship  both between human's and robots \cite{kim2009repair,miles1995organizational}, meaning first impressions are crucial for trust. First impressions from audio and visual stimulus can also damage the ability to develop trust later on \cite{Schaefer2016}. In this work we focus on affective trust, which is developed through emotional bonds and personal relationship, not competence \cite{freedy2007measurement}. Affective trust makes relationships more resilient to mistakes by either party \cite{rousseau1998not}. The display of emotion is critical for affective trust and increases the willingness of collaboration \cite{gompei2018factors}.

Music and prosody has been shown as a powerful medium to convey emotions \cite{sloboda1999music}. In music and robotics emotion can be categorized in many ways, such as a discrete categorical manner (happiness, sadness, fear, etc.) \cite{devillers2005challenges}, and through continuous dimensions such as valence, arousal \cite{russell2009emotion}. While some recent efforts to generate and manipulate robotic emotions through  prosody focused on linguistic robotic communication \cite{crumpton2016survey}, \cite{breazeal2002recognition}, there has only recently been work focusing on musical prosody \cite{savery_finding_2019,savery2019establishing}.







One of the main aims of the presented work concerns recovery of trust, which it assumes a loss of trust. I think the background could be extended by including a deeper discussion concerning trust and sounds, and the communication of errors. 




% \subsection{Musical Prosody} 
% One main reason we chose to investigate musical prosody as a feedback mechanism for human-robot interactions is to avoid the uncanny valley \cite{macdorman2006subjective}. Prosody has the potential to allow the robot to communicate in a manner relatable to that of humans, but still different from day to day human speech. Additionally, affective nonverbal behavior has been shown to affect humans' emotional state and self-disclosure when interacting with a robot, as well as their perceived animacy of the robot \cite{rosenthal2018effects}. Gestures have been explored for creating an affect space for robots \cite{beck2010towards}, but non-linguistic forms of audio feedback are under-explored. Sonification (turning data into sound) and non-speech audio feedback have been used to improve user performance in a variety of tasks \cite{hermann2011sonification}. Therefore, audio feedback is a good candidate to explore for these types of interactions. 

% WHY MUSICAL PROSODY
% - WHY USE MUSICAL PROSODY
% At the basis of the original choice to use musical prosody is a decision to avoid uncanny valley


% - AVOID UNCANNY VALLEY AND CREATE AN EMOTIONAL AGENT 
% builds on avoiding uncanney valley, by allowing a robot to communicate in a manner that is relatable to human communication, but different from day to day speech. Developing an emotional agent. 
% avoid uncanny valley leading to 


% - EMOTIONAL AGENT

% DISCUSS VARIATION IN COMPASSION AND HATE


% - Prosody makes sense as very low technical and financial cost.
% - Does not require changes to system
% - Sounds have been shown to not draw focus from core tasks (sonification paper)

% Avoid uncanny valley 

% % Images of music and description of data


